Interpretable Personalization via Policy Learning with Linear Decision Boundaries

With the rise of the digital economy and an explosion of available information about consumers, effective personalization of goods and services has become a core business focus for companies to improve revenues and maintain a competitive edge. This paper studies the personalization problem through the lens of policy learning, where the goal is to learn a decision-making rule (a policy) that maps from consumer and product characteristics (features) to recommendations (actions) in order to optimize outcomes (rewards). We focus on using available historical data for offline learning with unknown data collection procedures, where a key challenge is the non-random assignment of recommendations. Moreover, in many business and medical applications, interpretability of a policy is essential. We study the class of policies with linear decision boundaries to ensure interpretability, and propose learning algorithms using tools from causal inference to address unbalanced treatments. We study several optimization schemes to solve the associated non-convex, non-smooth optimization problem, and find that a Bayesian optimization algorithm is effective. We test our algorithm with extensive simulation studies and apply it to an anonymized online marketplace customer purchase dataset, where the learned policy outputs a personalized discount recommendation based on customer and product features in order to maximize gross merchandise value (GMV) for sellers. Our learned policy improves upon the platform's baseline by 88.2\% in net sales revenue, while also providing informative insights on which features are important for the decision-making process. Our findings suggest that our proposed policy learning framework using tools from causal inference and Bayesian optimization provides a promising practical approach to interpretable personalization across a wide range of applications.

==> logistic_class.tex <==
\section{Logistic Policy Class }

\subsection{Logistic Policy}

Instead of argmax linear policy with the so-called softmax linear
policies, i.e. instead of selecting the policy corresponding to the
largest entry of the linear function, we apply a logistic transformation
to obtain a random policy. 

Similar to convex relaxation, this approach relaxes the objective
function so that it becomes differentiable. However, instead of seeking
a convex lower bound of the objective, we directly replace the policy
obtained from argmax of linear function with policy obtained from
softmax of linear function, i.e. apply a logistic transformation to
obtain randomized policies. More precisely, given parameters $\Theta$
and data $X$, the class of randomized linear policies is represented
by 
\begin{align*}
\pi(\Theta,X_{i}) & =\begin{bmatrix}\frac{\exp(\Theta_{1}^{T}X_{i})}{\sum_{j}\exp(\Theta_{j}^{T}X_{i})}\\
\vdots\\
\frac{\exp(\Theta_{p}^{T}X_{i})}{\sum_{j}\exp(\Theta_{j}^{T}X_{i})}
\end{bmatrix}
\end{align*}

The solution of the optimization problem over this different class
of policies does not yield a lower bound on the objective, but its
advantage is that it is differentiable and so we may directly apply
gradient descent in the optimization step. In fact, in practice argmax
is rarely employed precisely because of the fact that it is non-differentiable.
Empirical performance of softmax optimization shows that its decision
boundaries are very similar to argmax linear policies. 

\subsection{Complexity Bound}

\subsection{Experiments}

\begin{figure}
\begin{centering}
\includegraphics[scale=0.3]{\string"Logistic Class/logistic_nonlinear_2d_opt\string".png}\includegraphics[scale=0.3]{\string"Logistic Class/logistic_nonlinear_2d_0\string".png}
\par\end{centering}
\begin{centering}
\includegraphics[scale=0.3]{\string"Logistic Class/logistic_nonlinear_2d_AIPW_2\string".png}\includegraphics[scale=0.3]{\string"Logistic Class/logistic_nonlinear_2d_IPW_2\string".png}
\par\end{centering}
\caption{Left to right, top to bottom: Optimal decision boundary; logistic
policy with mean expected rewards; logistic policy with AIPW estimator;
logistic policy with IPW estimator. Sample size is 2500, variance
is 4, dimension is 2D.}
\end{figure}

\begin{figure}
\begin{centering}
\includegraphics[scale=0.3]{\string"Logistic Class/logistic_nonlinear_2d_opt\string".png}\includegraphics[scale=0.3]{\string"Logistic Class/nn_1_nonlinear_2d_0\string".png}
\par\end{centering}
\begin{centering}
\includegraphics[scale=0.3]{\string"Logistic Class/nn_1_nonlinear_AIPW_2\string".png}\includegraphics[scale=0.3]{\string"Logistic Class/nn_1_nonlinear_IPW_2\string".png}
\par\end{centering}
\caption{Left to right, top to bottom: Optimal decision boundary; 1 hidden
layer neural net with mean expected rewards; 1 hidden layer neural
net policy with AIPW estimator; 1 hidden layer neural net policy with
IPW estimator. Sample size is 2500, variance is 4, dimension is 2D.}
\end{figure}

\begin{figure}
\begin{centering}
\includegraphics[scale=0.3]{\string"Logistic Class/logistic_nonlinear_2d_opt\string".png}\includegraphics[scale=0.3]{\string"Logistic Class/nn_2_nonlinear_2d_0\string".png}
\par\end{centering}
\begin{centering}
\includegraphics[scale=0.3]{\string"Logistic Class/nn_2_nonlinear_AIPW_2\string".png}\includegraphics[scale=0.3]{\string"Logistic Class/nn_2_nonlinear_IPW_2\string".png}
\par\end{centering}
\caption{Left to right, top to bottom: Optimal decision boundary; 2 hidden
layer neural net with mean expected rewards; 2 hidden layer neural
net policy with AIPW estimator; 2 hidden layer neural net policy with
IPW estimator. Sample size is 2500, variance is 4, dimension is 2D.}
\end{figure}

\begin{table}
\begin{centering}
\begin{tabular}{|c|c|c|c|c|c|}
\hline 
\multicolumn{2}{|c|}{training set size} & \multicolumn{2}{c|}{2500 samples} & \multicolumn{2}{c|}{15000 samples}\tabularnewline
\hline 
\multicolumn{2}{|c|}{value of optimal policy} & \multicolumn{2}{c|}{2.26} & \multicolumn{2}{c|}{2.26}\tabularnewline
\hline 
\multicolumn{2}{|c|}{noise variance of observed data} & $\sigma^{2}=4$ & $\sigma^{2}=36$ & $\sigma^{2}=4$ & $\sigma^{2}=36$\tabularnewline
\hline 
\hline 
\multirow{2}{*}{logistic (softmax)} & AIPW & 2.02 & 1.82 & 2.02 & 1.98\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & IPW & 2.01 & 1.76 & 2.01 & 1.98\tabularnewline
\hline 
\multirow{2}{*}{1-hidden layer nn (softmax)} & AIPW & 2.05 & 2.05 & 2.08 & 2.02\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & IPW & 2.02 & 2.12 & 2.06 & 1.97\tabularnewline
\hline 
\multirow{2}{*}{2-hidden layer nn (softmax)} & AIPW & 2.18 & 2.03 & 2.04 & 1.95\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6} 
 & IPW & 2.16 & 1.99 & 2.04 & 2.08\tabularnewline
\hline 
\end{tabular}
\par\end{centering}
\caption{Values of trained policies using AIPW and IPW estimators of potential
rewards for the nonlinear simulated dataset.}
\end{table}

==> theory.tex <==
\section{Theoretical Guarantees}
\label{sec:theory}

In this section, we provide a general connection between the entropy integral \citep{dudley1967sizes} of a function class and two generalizations of the VC dimension \citep{vapnik1971uniform} to higher dimensions, and then specialize it to prove the $\mathcal{O}_p(1/\sqrt{n})$ optimal regret bound for policies with linear decision boundaries solving the ERM problem \eqref{eq:ERM} with doubly robust reward estimators \eqref{eq:AIPW}.  Regret bounds for additional policy classes that are popular in practice, such as random forests and neural networks, can be found in Appendix \ref{app:additional}. Proofs of all results can be found in Appendix \ref{app:proofs}.

\subsection{Complexity Measures of a Policy Class}
 We measure the complexity of a multi-action policy class by its graph dimension and Natarajan dimension, two generalizations of the VC dimension. 
Given $\feas$, a deterministic policy class
$\Pi$,  and a set of data points
$S=\{x_{1},\dots,x_{n}\} \subset \feas , n \ge 1$ , let $\Pi(S)$ denote the set of all possible outcomes of $\Pi$ acting on $S$, i.e. 
\begin{equation}
   \Pi(S) = \left\{ \left(
(\pi(x_1), \dots, \pi(x_n))|\pi \in \Pi
\right)  \right\} \subset \actions^n. 
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Graph dimension %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}\label{def:graph_dim_policy}(Graph dimension)\quad  
We say a set $V \subset \actions^n$ G-shatters an index set $I\ \subset \{1,\dots, n\}$ if there exists some function $f: I \to \actions$ such that $\forall J \subset I$, $\exists v \in V$ such that $\forall i \in J,  v_i =f(i); \forall i \in I/J,  v_i \neq f(i).$
The graph dimension of $V$, denoted by $\gdim(V)$, is the maximal size of index set shattered by $V$.
The \textbf{graph dimension} of $\Pi$ is:
\begin{equation}
    \gdim(\Pi) \;:=\; \sup_{\text{finite } S \subset \feas} \gdim(\Pi(S))
\end{equation}
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Natarajan dimension of a set %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}\label{def:Natarajan_dim_policy}(Natarajan dimension)\quad  
We say a set $V \subset \actions^n$ N-shatters an index set $I\ \subset \{1,\dots, n\}$ if there exist $f_1, f_2: I \to \actions$ such that
$\forall J \subset I$, $\exists v \in V$ such that $ \forall i \in J,  v_i =f_1(i);\forall i \in I/J,  v_i =f_2(i).$
The Natarajan dimension of $V$, denoted by $\ndim(V)$, is the maximal size of index set shattered by $V$. 
The \textbf{Natarajan dimension} of $\Pi$ is:
\begin{equation}
    \ndim(\Pi) \;:=\; \sup_{\text{finite } S \subset \feas} \ndim(\Pi(S))
\end{equation}
\end{definition}

\textbf{Remark.} The graph and Natarajan dimensions capture the complexity of a policy class through the cardinality of outcomes that its elements are able to discriminate. When there are exactly two possible actions, i.e. $d=2$, $\gdim(\Pi) = \ndim(\Pi)= \vcdim(\Pi)$. Therefore, both the graph dimension and the Natarajan dimension generalize the VC dimension. Natarajan dimension and graph dimension differ at most by a  factor of log number of actions. In~\cite{ben-david1995characterizations} it was proved that for every policy class $\Pi \subseteq \actions^{\feas}$ ,
\begin{equation}\label{eq:relationship_of_ndim_and_gdim}
    \ndim(\Pi) \le \gdim(\Pi) 
    \le 4.67 \log_2 \left(|\actions|\right)\ndim(\Pi).
\end{equation}

We next introduce the entropy integral. We start with some basic concepts.

\begin{definition} %(Hamming distance of two vectors in $\actions^n$) \quad
Fix any $n\ge 1$. 
\begin{enumerate}
    \item 
The \textbf{Hamming distance} between any two vectors $u,v$ in $\mathcal{A}^n$ is $H(u,v)=\frac{1}{n}\sum_{i=1}^n {\rm \mathbf 1}_{\{u_i\neq v_i\}}$.
 %($\epsilon$-covering and covering number of $V \subset \actions^n$) \quad
A set $\{v_1, ..., v_N \} \subset \actions^n $ is an $\epsilon$-covering of $V \subset \actions^n $ if for any $v \in V$, there exist an $v_i$ such that $H(v, v_i) \le \epsilon$. The \textbf{$\epsilon$-covering number} of $V$, denoted by $\covering(\epsilon, V)$, is the smallest number $N$ such that there exist an $\epsilon$-covering of $V$ of size $N$.
% ($\epsilon$-packing and packing number of some $V \subset \actions^n$) \quad
\item
A set $\{v_1, ..., v_M \} \subset V$ is an $\epsilon$-packing of $V \subset \actions^n $ if for all $i\neq j$, $H(v_i, v_j) \ge \epsilon$. The \textbf{$\epsilon$-packing number} of $V$, denoted by $\packing(\epsilon, V)$, is the largest number $M$ such that there exist an $\epsilon$-packing of $V$ of size $M$.
\end{enumerate}
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Covering and packing equivalence %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The packing number and covering number are related (\cite{wainwright2019highdimension}): 
\begin{equation}\label{eq:covering_and_packing_set}
\forall V \subset \actions^n,    \packing(2\epsilon, V) \le \covering(\epsilon, V) \le \packing(\epsilon, V).
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Covering number of a policy class %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition} \label{def:entropy_integral}
The $\epsilon$-covering number of $\Pi$ is $\covering(\epsilon,\Pi) \; = \; \sup_{\text{finite } S \subset \feas} \covering(\epsilon,\Pi(S)).$
The \textbf{entropy integral} of a policy class $\Pi$ is $\ei(\Pi) = \int_0^1 \sqrt{\log\covering(\epsilon^2, \Pi)} \; d\epsilon$.
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Assumption 3 %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Note that the covering number as defined above is a classical notion (see~\cite{maurer2009empirical} for a detailed treatment). Under a mild growth assumption on the covering number that guarantees the entropy integral is finite, the regret of a policy $\ipw$ solving the ERM problem with AIPW estimators can be bounded by entropy integral of the policy class $\Pi$ with high probability (\cite{zhou2018offline}, Theorem 3): 
\begin{equation} \label{eq:regret_by_ei}
   R_{\Pi}(\ipw) = \mathcal{O}_p 
   \left(
   \ei(\Pi)\sqrt{\frac{V_{*}}{n}} 
   \right),
\end{equation}
where
$V_* := \sup_{\pi_a, \pi_b \in \Pi}\E[\langle\Gamma_i, \pi_a(X_i) - \pi_b(X_i)\rangle^2]$ can be interpreted as the worst-case variance of evaluating the difference 
	between two policies in $\Pi$.	
	\begin{comment}
		: it measures how variable it is to evaluate the difference between
		$\langle\Gamma_i, \pi_a(X_i) \rangle$ (the policy value when using $\pi_a$) and $\langle\Gamma_i, \pi_b(X_i)\rangle$ (the policy value when using $\pi_b$) in the worst-case. Intuitively, the more difficult it is to evaluate this worst-case difference (i.e. the larger the $V_*$), the harder it is to distinguish between two policies, and hence the larger the (Rademacher) complexity.
	\end{comment} 
In binary-action policy learning ($d = 2$), using a bound of \cite{haussler1995sphere} on the packing number by VC dimension,
\begin{equation} \label{eq:packing_bound_VC}
\packing(\epsilon, V) 
\;\le \; e(\vcdim(V) + 1) \left(\frac{2e}{\epsilon}\right)^{\vcdim(V)}
\end{equation}
for any $V \subset \{0,1\}^n$, one can further show that $\ei(\Pi) \le 2.5 \sqrt{\vcdim(\Pi)}$. Plugging into the regret bound by entropy integral in \eqref{eq:regret_by_ei}, we have 
$R_{\Pi}(\ipw)  = \mathcal{O}_p\left( \sqrt{\frac{V_* \cdot \vcdim(\Pi)}{n}} \right)$. For multi-action policies ($d>2$), however, there does not exist a meaningful bound for the entropy integral of a function class in general, as the VC dimension only applies to $d=2$. We now solve this problem by providing a bound of $\ei(\Pi)$ by the \emph{graph} dimension of a function class when $d>2$, which will then allow us to prove the optimal regret bound for policies with linear decision boundaries.

\begin{comment}
	\cite{haussler1995sphere}
	shows that the packing number can be bounded by VC dimension as follow: for any $V \subset \{0,1\}^n$,
	\begin{equation} \label{eq:packing_bound_VC}
	\packing(\epsilon, V) 
	\;\le \; e(\vcdim(V) + 1) \left(\frac{2e}{\epsilon}\right)^{\vcdim(V)}.
	\end{equation} 
	We can see that this inequality also holds for $V$ substituted by any binary-action policy class $\Pi$. Since the covering number is bounded by the packing number, we have 
	\begin{equation}\label{eq:covering_bound_VC}
	\covering(\epsilon, \Pi) \le e(\vcdim(\Pi) + 1) \left(\frac{2e}{\epsilon}\right){\vcdim(\Pi)}.
	\end{equation}
	From here, by taking the natural log of both sides and computing the entropy integral, one can show that $\ei(\Pi) \le 2.5 \sqrt{\vcdim(\Pi)}$. Plugging into the regret bound by entropy integral in \eqref{eq:regret_by_ei} , we have 
	$R(\ipw)  = O_p\left( \sqrt{\frac{V_* \cdot \vcdim(\Pi)}{n}} \right)$
\end{comment} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% Theorem: Graph dim bound packing number %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}
\label{thm: ei_bound_by_gdim} \quad For any policy class $\Pi$,
% \begin{equation}\label{eq:packing_bound_graph}
%      \packing(\epsilon, \Pi) 
%     \;\le \; e(\gdim(\Pi) + 1) \left(\frac{ed}{\epsilon}\right)^{\gdim(\Pi)}.
% \end{equation}
\begin{equation}\label{eq:ei_bound_graph}
\ei(\Pi)\leq 	\mathcal{O}(\log d\cdot \gdim(\Pi)) = \mathcal{O}\big((\log d)^2\cdot \ndim(\Pi)\big) .
\end{equation}

\end{theorem}

Using the bound on the entropy integral in Theorem~\ref{thm: ei_bound_by_gdim}, we can 
%Using the bound on the packing number obtained in Theorem \ref{thm: covering_bound_by_gdim}, we can bound the entropy integral of linear decision boundaries and then 
apply the regret bound from \cite{zhou2018offline} to obtain the optimal regret bound for policies with linear decision boundaries solving the ERM problem \eqref{eq:ERM} with AIPW reward estimators. We require estimators of the propensity and reward models satisfy the following consistency assumption \citep{athey2017efficient,zhou2018offline}:
\begin{assumption}
	\label{assump:consistency}Let $\hat{e}_{a^{j}}(x)$ and $\hat{\mu}_{a^{j}}(x)$
	denote cross-fitted estimators of propensity scores and expected rewards used in the AIPW estimator in \eqref{eq:AIPW}. They satisfy the following error
	bounds:
	\begin{align}
	\mathbb{E}\left[(\hat{\mu}_{a^{j}}(X)-\mu_{a^{j}}(X))^{2}\right]\cdot\mathbb{E}\left[(\hat{e}_{a^{j}}(X)-e_{a^{j}}(X))^{2}\right] & =\frac{o(1)}{n},\forall a^{j}\in\mathcal{A} \label{eq:consistency}
	\end{align}
\end{assumption}
In general, provided $\mu_{a}(\cdot)$ and $e_{a}(\cdot)$ are sufficiently
smooth, Assumption \ref{assump:consistency} is often satisfied by estimators from the statistical estimation literature.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% Regret bound by Graph dimension %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem} \label{regret bound} 
        Under Assumptions~\ref{assump:classical} and \ref{assump:consistency} and for general policy class $\Pi$,
        \begin{equation}
            R_{\Pi}(\ipw) = \mathcal{O}_p\left( \sqrt{\frac{V_* \cdot \log d \cdot \gdim(\Pi)}{n}} \right) = \mathcal{O}_p\left( \sqrt{\frac{V_* \cdot (\log d)^2 \cdot \ndim(\Pi)}{n}} \right)
        \end{equation}  
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% examples %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% Examples to calculate graph dimension to bound regret %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next we apply this bound to the class $\Pi_{\text{linear}}$ of policies with linear decision boundaries, which have known graph dimension. 
%\textbf{Linear decision boundaries.} The class $\Pi_{\text{linear}}$ of policies with linear decision boundaries 
%have known graph dimension. 
\begin{lemma}
(\cite{daniely2012multiclass}) The graph dimension of policies with linear decision boundaries is $\mathcal{O}(dp \log(dp))$.
\end{lemma}
With this characterization, we apply Theorem \ref{regret bound} to give the main minimax optimality result for linear decision boundary policies:
\begin{theorem} (\textbf{Main Regret Bound for Linear Decision Boundary Policies}) 
 Let $\ipw \in \linear$ be the linear decision boundary policy learned from the ERM problem \eqref{eq:ERM} and let Assumptions~\ref{assump:classical} and \ref{assump:consistency} hold. Then, 
$R_{\linear}(\ipw) = \mathcal{O}_p\left(\sqrt{\frac{V_* \cdot dp  \log d\log dp }{n}} \right)$. 
In particular, for fixed $p$ and $d$, $R(\ipw) = \mathcal{O}_p\left(\sqrt{\frac{V_* }{n}} \right)$.
\end{theorem}

Compared to the regret upper bound obtained in \cite{zhou2018offline} through exact computation of the entropy integral, our upper bound has a higher order of $\log d$, the logarithm of the number of actions. However, our approach via the graph dimension provides a more disciplined way to establish regret upper bounds for a broad range of policy classes, while the original bound by entropy integral in \cite{zhou2018offline} might provide slightly tighter bounds in special cases.  In Appendix \ref{app:additional}, we apply the general result in Theorem \ref{regret bound} to additional policy classes, including tree-based policies, neural networks with ReLU activations, and random forests, which are widely used in practice.
